The Creation and Detection of Deepfakes: A Survey

Generative deep learning algorithms have progressed to a point where it is difficult to tell the difference between what is real and what is fake. In 2018, it was discovered how easy it is to use this technology for unethical and malicious applications, such as the spread of misinformation, impersonation of political leaders, and the defamation of innocent individuals. Since then, these `deepfakes' have advanced significantly. In this paper, we explore the creation and detection of deepfakes and provide an in-depth view of how these architectures work. The purpose of this survey is to provide the reader with a deeper understanding of (1) how deepfakes are created and detected, (2) the current trends and advancements in this domain, (3) the shortcomings of the current defense solutions, and (4) the areas which require further research and attention.

==> sec_reenactment_bak1.tex <==

	[table: reenactment summary - general]
	
	[table: reenactment summary - training/datasets]
	
	[fig: reenactment schematics]
	
	%\subsection{Facial Reenactment}
	First we will review facial reenactment and then body reenactment
	
	\subsection{Expression Reenactment}\label{subsec:expression}
	In news and popular culture, one of the most common type of deepfake is expression reenactment. This is because it gives attackers the most flexibility in producing content with the desired impact, turning their victim's identity into a puppet. However, expression reenactment has been around long before deepfakes were popularized. In 2003, researchers showed how this is possible by 3D scanning the source and then morphing a 3D model of the target's image accordingly \cite{blanz2003reanimating}. In 2005, it was shown how this can be done without a 3D model \cite{chang2005transferable}. Later, between 2015 and 2018, Thies et al. demonstrated how RGB-D (depth sensing) cameras can be used to create real-time reenactments using 3D parametric models to achieve high quality results \cite{thies2015real,thies2016face2face,thies2018headon}. 
	
	Aside from realism, a key aspect to deepfake technologies is their practicality. For example, researchers have been working on ways to limit the amount of target specific data required for reenactment. In the following subsections, we present a chronological review these works according to their class of generalization. 

%\vspace{1em}	
%\noindent\textbf{Identity to Identity (One-to-One).}
\subsubsection{\textbf{Identity to Identity (One-to-One)}}
	\emph{Initial Works.} One of the first works to use deep learning for expression reenactment was in 2017 in \cite{bao2017cvae}. There authors propose CVAE-GAN, a conditional VAE-GAN where the generator is conditioned on an attribute vector or class label. In their evaluations, the authors briefly show how the network can be used for attribute morphing by interpolating the latent variables (e.g., between target poses).
	Later, the authors of \cite{xu2017face} proposed the use the popular CycleGAN architecture \cite{zhu2017unpaired} for this task. Using two sets of video frames (domains) one for $s$ and one for $t$ the authors were able to train model without the need for image paring during training (e.g., two identities with the same expression). However, to avoid artifacts in $x_g$, both domains must share a similar distributions (e.g., poses and expressions).
	
	\emph{Temporal GANs.} In 2018, Bansal et al. proposed a generic translation network based on CycleGAN called Recycle-GAN \cite{bansal2018recycle}. Their framework improves temporal coherence and mitigates artifacts by including next-frame predictor networks for each domain. For facial reenactment, the authors train their network to translate the facial landmarks of $x_s$ to talking portraits of $x_t$.
	In \cite{tulyakov2018mocogan}, the authors propose MoCoGAN: a temporal GAN which generates videos by disentangling the motion and content (objects). Each frame is produced with a decoder using a target expression label $z_c$, and a motion embedding $z_{M}^{(i)}$ for the $i$-th frame, obtained from a noise seeded RNN. MoCoGAN uses two discriminators, one for realism  (per frame) and one for temporal coherence (on the last $T$ frames). 

	

\subsubsection{\textbf{Multiple Identities to a Single Identity (Many-to-One)}}\label{subsubsec:expression:many2one}
	In 2018, researchers aimed to make facial reenactment practical with source-identity agnostic models. Initially, focus was placed on decoupling the dependency between a set of source identities and a target's identity: %\footnote{Although works such as \cite{olszewski2017realistic} and \cite{zhou2017photorealistic} achieved fully agnostic models (many-to-many) in 2017, their works are on low res or partial faces}
	
	\emph{Facial Boundary Conversion.}
	In \cite{wu2018reenactgan}, the authors attempted to decouple the source identity by passing the generator an embedding of source's facial boundaries ($b_s$) instead of the image. Their framework `ReenactGAN' uses a CycleGAN to transform $b_s$ to the target face shape as $b_t$ before generating $x_g$ using a pix2pix-like generator.	
	
	\emph{Temporal GANs.}
	In \cite{wang2018vid2vid}, the authors proposed a framework called Vid2Vid, similar to pix2pix but for videos. Vid2Vid considers the temporal aspect by generating each frame based on the last $L$ source and generated frames. The model also considers next-frame occlusion prediction and optical flow. A progressive training strategy is used on the resolution and frame rate to produce high quality results. In their evaluations, the authors demonstrate facial reenactment using the source's facial boundaries.
	In \cite{kim2018deep}, the authors achieved complete facial reenactment (gaze, blinking, pose, mouth, etc.) with one minute of a target's video using a GAN. Their approach was to extract the source and target's 3D facial models from 2D images using monocular reconstruction \cite{zollhofer2018state}, and then for each frame, (1) transfer the facial pose and expression of the source's 3D model to the target's, and (2) produce $x_{g}$ with a modified pix2pix framework, using the last 11 frames of rendered heads, UV maps, and gaze masks as the input.

\subsubsection{\textbf{Multiple Identities to Multiple Identities (Many-to-Many)}}\label{subsubsec:expression:many2many}

	\emph{Initial Works.} The first attempts at a source and target agnostic model were in 2017, where the authors of \cite{olszewski2017realistic} used a conditional GAN (CGAN) for the task. Their approach was is to extract and concatenate the UV-normalized inner-face regions as $(x_t,x_s)$, and then pass them an ED to produce $x_g$ which is subjected to adversarial and L1 loss. The challenge of using a CGAN is that the training data must be paired (images of different identities with the same expression). %The authors solved this problem by using a custom dataset of multiple actors performing the same activities.
	Going one step further, in \cite{zhou2017photorealistic} the authors reenacted full portraits albeit at low resolutions. Their approach to achieving an agnostic model was to disentangle the identity from the expression in the latent space of a conditional adversarial autoencoder. However, the approach was limited to driving $x_t$ with discreet AU expression labels that capture $x_s$. A similar label based reenactment was presented in the evaluation of StarGAN \cite{choi2018stargan}; an architecture similar to CycleGAN but for $N$ domains (poses, expressions, etc).
	
	%\vspace{0.5em}
	Later, in 2018, the authors of \cite{pham2018generative} proposed GATH which can drive $x_t$ using continuous action units (AU) as an input, extracted from $x_s$. Their generator is ED network trained on the loss signals from using three other networks: (1) a discriminator, (2) an identity classifier, and (3) a pretrained AU estimator. The classifier shares the same hidden weights as the discriminator disentangle the identity from the expression. 
	

	\emph{Self-Attention Modeling.}
	%**
	Similarly, another work called GANimation \cite{pumarola2019ganimation} reenacts faces through AU value inputs, estimated from $x_s$. Their architecture uses a generator transforms a face according to an AU vector, and uses a self attention model to handle occlusions, and mitigate other artifacts. Furthermore, a WGAN-GP inspired discriminator is used to evaluate the image quality and another network, with some shared weights with the discriminator, is used to penalize errors in the generated expression. Similar to CycleGAN, GANimation uses a cycle consistency loss which eliminates the need for image pairing.	
	%*
	Instead of relying on AU estimations, in \cite{sanchez2018triple} the authors propose GANnotation which generates $x_g$ based on $(x_t,l_s)$, where $l_s$ is the facial landmarks of $x_s$. GANnotation uses that same self attention model as GANimation, but proposes a novel ``triple consistency loss'' to minimize artifacts in $x_g$ by learning how to deal with intermediate poses/expressions not found in the training set. Given $l_s,l_t$ and $l_z$ sampled randomly from the same video, the loss is computed as $\mathcal{L}_{trip}=\|\|G(x_t,l_s)-G(G(x_t,l_z),l_s)\|\|^2$

	\emph{3D Parametric Approaches.}
	%**	
	Concurrent to the work of \cite{kim2018deep}, other works also leveraged 3D parametric facial models to prevent identity leakage in the generation process.
	In \cite{shen2018faceid}, the authors propose FaceID-GAN which works at oblique poses and high resolution. Their ED generator is trained in tandem with a 3DMM parametric face model predictor, where the parameters $x_s$ is used to transform the parameters of $x_s$ before being joined with the encoder's embedding. Furthermore, to prevent identity leakage from $x_s$ to $x_g$, FaceID-GAN incorporates an identification classifier within the adversarial game. The classifier has $2N$ outputs where the first $N$ outputs (corresponding to training set identities) are activated if the input is real and the rest are activated if it's fake.
	%*
	Later, the authors of \cite{shen2018faceid} propose FaceFeat-GAN which improves the diversty of the faces while preserving the identity \cite{shen2018facefeat}. In FaceFeat-GAN, three encoder/predictor neural networks $P$, $Q$, and $I$, are trained on real images to extract feature vectors from portraits. $P$ predicts 3DMM parameters $p$, $Q$ encodes the image as $q$ capturing general facial features using feedback from $I$, and $I$ is an identity classifier trained to predict label $y_i$. Next two GANs, seeded with noise vectors, produce $p'$ and $q'$ while a third GAN is trained to reconstruct $x_t$ from $(p,q,y_i)$ and $x_g$ from $(p',q',y_i)$. To reenact $x_t$, (1) $y_t$ is predicted using $I$ (even if the identity was previously unseen), (2) $z_p$ and $z_q$ are selected empirically to fit $x_s$, and (3) the third GAN's generator uses $(p',q',y_t)$ to create $x_g$. 
	%
	In \cite{nagano2018pagan}, the authors present paGAN, a method for complete facial reenactment on a 3D avatar, using a single image of the target as input. With an image of $x_t$ in a neutral expression, the authors drive the extracted 3D model with $x_s$ and obtain the rendered head with its UV map and depth map. Finally, these inputs including references to the target's eye and face, are used by a U-Net AE to generate a refined texture for the 3D model. The gaze is controlled by masking the eyes in the rendered face and placing white points where the pupil should be (via in-painting).
	
	\emph{Using Multi-Modal Sources.}
	%**
	In \cite{wiles2018x2face} the authors propose X2Face which reenacts a portrait using another portrait or some other modality such as audio or a pose vector. X2Face uses two ED networks: an embedding network and a driving network. First the embedding network encodes 1-3 examples of the target's face to $v_t$: the optical flow field required to transform $x_t$ to a neutral pose and expression. Next, $x_t$ is interpolated according to $m_t$ producing $x_{t}^{'}$. Finally, the driving network maps $x_s$ to the vector map $v_s$, crafted to interpolate $x_{t}^{'}$ to $x_g$, having the pose and expression in $x_s$. All interpolation is performed with a tensorflow interpolation layer to enable back propagation using $x_{t}^{'}$ and $x_g$.
	

	%\cite{yang2018pose} %uses class label to animate
	%reeenactment. need summary
	%\vspace{0.5em}
	In 2019, nearly all works focused on models which can be applied to new identities (source and target) unseen in the training data: 	

	\emph{Facial Landmark \& Boundary Conversion.}
	In \cite{zhang2019faceswapnet}, the authors propose FaceSwapNet which tries to mitigate the issue of identity leakage when facial landmarks are used.  First two encoders and a decoder are used to transfer the expression in landmark $l_s$ to the face structure of $l_t$, denoted $l_g$. Then a generator network is used to convert $x_t$ to $x_g$ where $l_g$ is injected into the network with AdaIn layers like a Style-GAN \cite{karras2019style}. The authors found that it is crucial to use triplet perceptual loss with an external VGG network.
	%occlusions
	%MAY NEED TO CUT
	In \cite{nirkin2019fsgan}, the authors present FSGAN: a face swapping and facial reenactment model which can handle occlusions.	For reenactment a pix2pixHD generator receives $x_t$ and the source's 3D facial landmarks $l_s$, represented as a 256x256x70 image (one channel for each of the 70 landmarks). The output $x_g$ and its segmentation map $m_g$ with three channels (background, face, and hair). The generator is trained recurrently where each output is passed back as input for several iterations while $l_s$ is interpolated incrementally from $l_s$ to $l_t$. To better match the target's pose, images of the source are queries with Delaunay Triangulation, and new images are generate with barycentric coordinate interpolation. In their evaluations they achieve real time reenactment at 30fps.
	In \cite{fu2019high}, the authors propose a method for high resolution reenactment and at oblique angles. A set of networks encode the source's pose, expression, and target's boundary. Then a decoder generates the target's boundary $b_g$ given this information. Finally, an ED network generates $x_g$ using an encoding of $x_t$'s texture in its embedding. Multi-scale loss is used to improve quality and the authors utilize a small labeled dataset by training their model in a semi-supervised way.

	\emph{Latent Space Manipulation.}
	In \cite{tripathy2019icface}, the authors presented a model called ICFace where the expression and pose can be driven independently. Their architecture is similar to a CycleGAN in that one generator translates $x_t$ into a neutral expression domain as $x_{t}^{\eta}$ and another generator translates $x_{t}^{\eta}$ into an expression domain as $x_g$. The first generator is conditioned with a neutral AU vector, and the second is conditioned with $x_s$'s AU vector. In their evaluation the authors showed how with this approach they can drive a target's expression, pose, mouth, eye, and eyebrows separately from a $x_s$.
	In \cite{qian2019make} the authors propose Additive Focal Variational Auto-encoder (AF-VAE) for high quality reenactment. This is accomplished by separating a C-VAE's latent code into an appearance encoding $e_a$ and identity-agnostic expression coding $e_x$. To capture a wide variety of factors in $e_a$ (e.g., age, illumination, complexion, ...), the authors proposed an additive memory module for training which conditions the latent variables on a Gaussian mixture model, fitted to clustered set of facial boundaries. Subpixel convolutions were used in the decoder to mitigate artifacts and improve fidelity, and a human inception score was proposed in for deepfake evaluation.	
	
	\emph{Warp-based Approaches.}
	In the past, facial reenactment was done by warping the image $x_t$ to the landmarks $l_s$ \cite{elor2017bringingPortraits}. In \cite{geng2019warp}, the authors propose wgGAN which uses the same approach but creates high-fidelity facial expressions by refining the image though a series of GANs: one for refining the warped face and another for in-painting the occlusions (eyes and mouth). A challenge with wgGAN is that the warping process is sensitive to head motion (change in pose).
	In \cite{zhang2019one}, propose a system which also controls gaze. They (1) use a network to segment $x_s$, (2) encode the appearance of $x_t$, and then (3) produce $x_g$ with a decoder that receives the encoding as an input and the segmentation in the inner layers using SPADE residual blocks. The authors blend $x_g$ with a warped version, guided by the segmentation, to mitigate artifacts in the background.

	
	\emph{Motion-Content Decoupling.}
	In \cite{otberdout2019dynamic} the authors propose a GAN for smoother facial reenactments of faces with neutral expressions. The authors state that animations of facial landmarks, between the neutral expression and a target expression, can be described as temporal curves in 2D space, summarized as points on a spherical manifold by calculating their square-root velocity function (SRVF). A WGAN is used to complete this distribution given target expression labels, and a pix2pix GAN is used to convert the sequences of reconstructed landmarks into a video frames of the target.
	\cite{wang2020imaginator}	
	In contrast to MoCoGAN \cite{tulyakov2018mocogan}, the authors of \cite{wang2020imaginator} propose ImaGINator: a conditional GAN which fuses both motion and content, but with transposed 3D convolutions to capture the distinct spatio-temporal relationships. The GAN also uses static and temporal discriminators, and to increase diversity, the authors also train the temporal discriminator with some videos using the wrong label. A disadvantage of \cite{otberdout2019dynamic} and \cite{wang2020imaginator} is that they are label driven and produce videos with a set number of frames.
	In \cite{siarohin2019animating}, the authors propose Monkey-Net: a self supervised network for driving an image with an arbitrary video sequence. Similar to MoCoGAN \cite{tulyakov2018mocogan}, the authors decouple the source's content and motion. First a series of networks produce a motion heat map (optical flow) using the source and target's key-points, and then an ED generator produces $x_g$ using $x_s$ as an input, and the optical flow in its embedding.
	Later in \cite{NIPS2019_8935}, the authors extend Monkey-Net by improving the object appearance when large pose transformations occur. They accomplish this by (1) modeling motion around the keypoints using affine transformations, (2) updating the key-point loss function accordingly, and (3) having the motion generator predict an occlusion mask on the preceding frame for in-painting inference.

	
	\subsubsection{\textbf{Few-Shot Learning}}
	Towards the end of 2019 and into the beginning of 2020, researchers began looking to minimizing the amount of training data via one-shot and few-shot learning. 
	%** %***add example frame from video
	In \cite{zakharov2019few}, the authors propose model which uses one or more images of the target, and work well at oblique angles. Their method preserved the target's identity at a wide range of facial poses unseen in the training data. To accomplish this, the authors perform meta-transfer learning \cite{sun2019meta}, where the network is first trained on many different identities and then fine-tuned on the target's identity. Their network first obtains and identity encoding by averaging the encodings of $k$ sets of $(x_t,l_t)$. Then a pix2pix GAN is used to generate $x_g$ using $l_s$ as an input, and the identity encoding at the inner layers via AdaIN layers. However, the authors note that their method is sensitive to identity leakage.
	In \cite{wang2019fewshotvid2vid} the authors of Vid2Vid (Section \ref{subsubsec:expression:many2one}) extend their work with few-shot learning. Using a network weight generation module which utilizes an attention mechanism. The module learns to extract appearance patterns from a few sample $x_t$ which are injected into the video synthesis layers. 
	%***	
	In \cite{MarioNETte:AAAI2020}, the authors propose MarioNETte which alleviates identity leakage when the pose of $x_s$ is different than $x_t$. In contrast to other works which encode the identity separately or the use of AdaIN layers, the authors use an image attention block and target feature alignment. The attention block is similar to the ED attention transformer of \cite{vaswani2017attention} where the source's feature map is used to query the target's feature map, thus preserving the spatial information. Target feature alignment warps the target's low-level feature maps. This enables the model to better handle the differences between face structures. 
	Finally, the identity is also preserved using a novel landmark transformer inspired by \cite{blanz1999morphable}. 	
	
	\subsection{Mouth Reenactment (Dubbing)}
	In contrast to expression reenactment, mouth reenactment (a.k.a., video or image dubbing) is concerned with driving a target's mouth with a segment of audio.
	
	\subsubsection{\textbf{Multiple Identities to a Single Identity (Many-to-One).}}
	\emph{Obama Puppetry.}
	%***
	In 2017, the authors of \cite{suwajanakorn2017synthesizing} created a realistic reenactment former president Obama. This was accomplished by (1) using a time delayed RNN over MFCC audio segments to generate a sequence of mouth landmarks (shapes), (2) generate the mouth textures (nose and mouth) by applying a weighted median to similar mouth shaped via PCA-space similarity, (3) refine the teeth by transferring the high frequency details other frames in the target video, and (4) use dynamic programming to re-time the target video to match the source audio and blend the texture in.
	Later that year, the authors of \cite{kumar2017obamanet} presented ObamaNet. a network that reenacts an individual's mouth and voice using text as input. The process is (1) convert the text to audio using Char2Wav \cite{sotelo2017char2wav}, (2) generate a sequence of mouth-keypoints using a time-delayed LSTM on the audio, and (3) use a pix2pix network to perform in-painting on a target video frame, where the mouth masked and the mouth-keypoints are supplied.
	Later in 2018, Jalalifar et al. \cite{jalalifar2018speech} proposed a network that synthesizes the entire head portrait of Obama, and therefore does not require pose timing like \cite{suwajanakorn2017synthesizing, kumar2017obamanet}. First, a bidirectional LSTM coverts MFCC audio segments into sequence of mouth landmarks, and then a pix2pix like network generates frames using the landmarks and a noise signal. After training, the pix2pix network is fine-tuned using a single video of the target to ensure consistent textures.	
	
	\emph{3D Parametric Approaches.}
	%**
	Later on in 2019, the authors of \cite{fried2019text} proposed a method for editing a transcript of a talking head which, in turn, modifies the target's mouth and speech accordingly.
	The approach is to (1) align phenomes to $a_s$, (2) fit a 3D parametric head model to each frame of $X_t$ \cite{kim2018deep}, (3) blend matching phenomes to create any new audio content, (4) animate the head model using the respective frames used during the blending process, and (5) generate $X_G$ with a CGAN RNN \cite{wang2018high} using composites as inputs (rendered mouths placed over the original frame). 
	%***	
	The authors of \cite{thies2019neural} had a different approach: (1) animate a the reconstructed 3D head with predicted blend shape parameters from $a_s$ using the DeepSpeech model for feature extraction, (2) use Deferred Neural Rendering \cite{thies2019deferred} to generate the mouth region, and then (3) use a network to blend the mouth into the original frame. The authors found that their approach only requires 2-3 minutes of video of the target to produce very realistic results.

	\subsubsection{\textbf{Multiple Identities to a Multiple Identities (Many-to-Many).}}
	%\cite{liu2011realistic}
	%In this apper the authors perform video dubing with the smilign expression for facial reenactment. The target is recorded in a studio reading text with neutral and smiling expressions. Then the animated talking head is rendered by parsing new text/audio (from TTS) and matching it to the most approapraite mouth region in the corpus.
	%**not deep
	One of the first works to perform identity agnostic video dubbing was \cite{shimba2015talking}. There the authors used an LSTM to map MFCC audio segments to the face shape. The face shapes were represented as the coefficients of an active appearance model (AAM), which are then used to retrieve the correct face shape of the target. 
	
	In \cite{song2018talking}, the authors three discriminators to improve temporal coherence: on the frames, video, and lip-sync. Frames are generated by (1) encoding each MFCC audio segment $a_{s}^{(i)}$ and $x_t$ with separate encoders, (2) passing the encodings through an RNN, and (3) decoding the outputs as $x_{g}^{(i)}$ using a decoder.

	%***
	The authors in \cite{zhou2019talking} mitigate identity leakage by using EDs to generate disentangled speech and identity encodings with adversarial classifiers. Then, $x_{g}^{(i)}$ is produced by a GAN using $x_t$'s identity encoding and a speech encoding as inputs. Since the speech encoder is trained to project audio and video into the same latent space, $x_g$ can be generated using either modalities as a source.

	%**
	In \cite{jamaludin2019you}, the authors propose Speech2Vid which also uses separate encoders for audio and identity. However, to capture the identity better, the identity encoder $En_I$ uses a concatenation of five images of the target, and there are skip connections from the $En_I$ to the decoder. To blend the mouth in better, a third `context' encoder is used to encourage in-painting. Finally, a VDSR CNN \cite{kim2016accurate} is applied to $x_g$ to sharpen the image.
	
	%**
	In \cite{vougioukas2019end}, the authors propose a dubbing network which also generates facial expressions and blinking. The approach is to (1) encode the identity of $x_t$ as $e_I$, (2) encode each audio segment $a_{s}^{(i)}$ via a CNN-RNN encoder as $e_{a}^{(i)}$, and (3) generate $x_g$ with a stride transposed CNN decoder, with $(e_I,e_{a}^{(i)},z_^{(i)}$ where $z_^{(i)}$ is the output of a GRU-based temporal noise generator. The GAN uses a video discriminator with two RNNs (for audio and video).%When applying the L1 loss, thne authors focus on the lower half of the face to encourage better lip sync quality over facial expressions.
	Later in \cite{vougioukas2019realistic}, the same authors improve the temporal coherence by splitting the video discriminator into two: (1) for temporal realism in mouth to audio synchronization, and (2) for temporal realism in overall facial expressions. 
	Then in \cite{kefalas2019speech}, the authors tune their approach further by fusing the encodings (audio, identity, and noise) with a polynomial fusion layer as oppesed to simply concatenating the encodings together. doing so makes the network less sensitive to large facial motions compared to \cite{vougioukas2019realistic} and \cite{}.	
	

	
	\cite{chen2019hierarchical}
	The authors state that direct models are problematic since the model learns irrelivant correlations between the audiovisual signal and the speech content. To avoid this issue, the authors first learn a direct mapping from audio to facial landmarks, and then model the mapping from the landmarks to the target identity. The audio-to-landmark network is an LSTM which receives the audio MFCC features and a compressed PCA representation of the coressponding facial landmarks.
	% The LSTM outputs the corresponding seqeunce of predicted compressed facial landmarks which are then expanded to full facial landmarks. 
	The landmark-to-identity network uses a convolutional RNN (CRNN) to generate the target's images using the sequnce of generated landmarks and latent information about the target's face. The authors adapt the attention mechanism from [Ganimation] by disentangling the motion from the audiovisual-non-correlated regions. Doing so help generate static pixels in regions that are not correlated to audio, and vice versa.
	To mitigate jitter, the authors introduce a dynamic pixel-wise loss with an attention mechanism. In additon, to improve face synchronization, the authors propose a regression based discermiantor which considers both sequence and content information. 
	
	\cite{nakashima2020speech}
	The authors perform video dubbing where the source and target are the same person... mostly uses cgi. Not so mal oriented bc requires source to look and sound the same.
	
	%summarize and place in category by date (many-2-one,date)

	
	
	\cite{liu2020synthesizing}
	\cite{yu2019mining}

	
	\subsection{Pose Reenactment}
	\cite{hu2018pose}
	note: facial reenactment of pose alone has mostly been researched for the task of frontalization [][][]. Some works have researched pose driven manipualtion, usch as ....
	They use a U-Net to convert a concatenation of $x_t$, $l_t$, and $l_s$ into $x_g$ using two discerminators. One discerminator distinguashed between real/fake rotated heads given the real head at a neutral pose, and the other discerminator distiguishes between real/fake heads at the same pose, given their landmarks.
	***to be cited very breifly in text
	
	\cite{tran2018representation}
	The authors propsoe DR-GAN for facial reenactment of pose for the task of pose-invariant face recognition. To adjust the pose of $x_t$, the authors use an ED GAN which encodes $x_t$ as $e_t$, and then decodes $(e_t,p_s,z)$ as $x_g$, where $p_s$ is the sources pose vector and $z$ is a noise vector. The authors show that the quality of $x_g$ can be improves by averaging multiple examples of $e_t$ togetehr before passing it through the decoder.	***to be cited very breifly in text
	
	\cite{cao20193d}
	The auhtors propose a system of two GANS for facial pose reenactment. The first GAN convert the face $x_t$ to a frontalized face image $x_{t}^{(f)}$ and its UV corrispondance map $uv_{t}^{(f)}$. This Gan is trained though adversarail loss on real/fake frontalized portraits and the UV map recontruction loss based on a 3DMM model extraction of the face for the ground truth. Next the second GAN utilized an ED generator to converts $(x_{t}^{(f)},uv_{t}^{(f)})$ to $x_g$, where the encoding is concatenated with the source's angle before going through the decoder.
	***to be cited very breifly in text
	

	
	\subsection{Gaze Reenactment}
	Some works have looked into facial reenactment of only gaze [][][] for the purpose of touching up images. For example,...
	
	\cite{ganin2016deepwarp}
	The authors peform gaze reenactment. The authors convert a cropped eye $x_t$, its landmarks, and the source angle, to a flow (vector) field using a 2-scale CNN. The flow field is then applied to $x_t$ warp it to the source angle, resulting in $x_g$. The auhtors then correct the illumination of $x_g$ with a second CNN.
	
	\cite{kononenko2017photorealistic}
	
	\cite{yu2019improving}
	The authors propose the Gaze Redireciton Network (GRN) for gaze reenactment using an ED network with cycle consistency loss. First the target's cropped eye $x_t$ is encoded and concatentated with target's head pose encoding and the source gaze angle encoding. Then the decoder produces a warp feild which is applied to $x_t$ to produce $x_g$. To overcome the lack of training data and the challenge of sample pairing, the authors (1) pretrain their network on 3D sythesized examples, (2) further tune their network on real images, and then (3) fine tune their network on 3-10 examplesof the target."
	***to be cited very breifly in text
	
	\subsection{Body Reenactment}

	==== mentioed in expression section, can be used for body too: ===
	\cite{wang2018vid2vid}
	\cite{wang2019fewshotvid2vid}
	\cite{tulyakov2018mocogan}
	\cite{siarohin2019animating}
	\cite{NIPS2019_8935}
	
	%\vspace{1em}	
	\noindent\textbf{Identities to Identity (One-to-One).}
	In the work of Liu et al. (2019), the authors perform facial reenactment with the upper-body as well (arms and hands). reenactment which can control a target's facial expressions, arms, and hands n \cite{liu2019video},. For each source frame, the process is to (1) extract the facial AUs and pose as the vector $b_s$ and extract the upper body key points as the image $u_s$ using avalaible libraries, (2) normalize $u_s$ (denoted $u_g$) using the method in [everybody dance now] and use $b_s$ to generate the target's facial boundry image $b_g$ with a pix2pixHD GAN, (3) paste $b_g$ into the image $u_g$ to form $c_g$, (4) use another pix2pixHD GAN to generate $x_g$ from the concatenation of $c_g$ and the last $L$ generated images $x_{g}^{(t-1)},\dots x_{g}^{(t-L)}$. For temporal coherence, the authors employ a similar strategy as [everybodydancenow] by supplying the discerminator with $x_{g}^{(t)},\dots x_{g}^{(t-L)}$ and $c_{g}^{(t)},\dots c_{g}^{(t-L)}$. The last GAN is also trained with temporal smoothing, feature mathcing, and perceptual losses.
	***requires lots of source and target video footage
	
	%\vspace{1em}	
	\noindent\textbf{Multiple Identities to a Single Identity (Many-to-One).}
	
	\cite{liu2019neural}
	In this paper the authors perform body reenactment and try to overcome some of the artifacts which occur in [everybody dance now] such as in correct detectio of skeletons which leads to stretched limbds. In their approach, the authors first build a 3D character model of their target with photogrammetry software and then animate it with the source actor's motion capture [MonoPerfCap: Human Performance Capture from Monocular Video]. The rendered model is then used to generate a realistic body on a given background using a pix2pix model. The input to the generator is the rendered body and their depth maps partitioned, and the target background. The discerminator uses applies L1 attention between $x_g$ anf $x_t$ on the adversrail loss to help the generator focus on relivant details as opposed to elemetns such as the static background. Approximalty 12k frames are used to train new generator per target with the pix2pix network. A challenge is that the attacker would need to obtain 100 images of the target from multiple angles with the same open pose in order to generate the 3D mesh character.	
	

	
	\cite{aberman2019deep}
	In [everybidy dnce], the authors train on paired data [[[[check]]]] which does not generalize well to unseen poses leading to artifacts. In a concurrent work to [everybody dance now], the authors in this paper mitigate this issue by using an upaired training branch with many identities other than $s$ and $t$. This also result in a reduction of training data from result 20min to 2min. Their model is a DNN which takes a 3D pose \cite{cao2017realtime} as an input and generates an image of the target's body in the given pose. To train their DNN, they use a GAN with two discermiantors over two training stages. In the first stage, the generator is trained on pairs of the target's pose and orgional frame using a combined loss from a discerminator. The discerminator considers whether a pose is real or fake given the frame, and whether the generated image is real or fake based on the the pose. The loss from a pretrained VGG-19 network is included to improve texture quality. After a few epochs, the loss function is extended by adding the loss of another discerminator which considers temporal coherence to ensure that the generator can translate unseen poses. The additional loss includes (1) the error between the current generated frame and the previouly gneerated frame after warping the previously generated frame with an optical flow field, and (2) the discermiantor's adversarial loss on predicting whether or not the pose is real or not (uncoupled to the input frame). The GAn was trained using 3000 video frames taken from the target performign various activitities. 
	
	\cite{chan2019everybody}
	The authors propsoe a mehtod for body reeanctment (dance) using a pix2pix GAN archotecture with a custom loss function. To capture the actor's pose for the network to intrepet, the authors convert frames into stick figures by (1) usesing an existing pose detector to extract the 2D x, y joint coordinates, and then (2) using the coordinates to plot key points and limbs as colored lines. The authors then train their GAN where the generator receives the curent pose and generates the frame, and the discerminator (1) verifies the realsim of the imagery conditioned on the pose, and (2) verifies temporal coherehence of the current and last generated frames conditioned on the pose. The authors also include the loss objectives from pix2pixHD and a pretrained VGGNet to improve texture quality. After training the generator, the weights are frozen and an additional pix2pix GAN is trained on the face region alone to improve the realism of the face. The face GAN is trained on a concatentation a cropped face (generated / real) and the respective cropped stick figure, where the generator receives concatentions of fake images only and produces the residual image that is used to imrove the generated image. The GAN is trained on 8-30 minutes of video footage on the target performign acticitities (dancing). To use the trained generator, the process for each frame is to (1) extract the driver's pose, (2) normalize the pose to the target's body, (3) pass the normalized pose through the body generator, and (4) improve the face region by passing the face through the face GAN. 
	***The authors also propose a method for detecting fake videos. They train a detector based on two consequtive frames which is trained in parralel to their GAN's sythesis process.
	
	%\vspace{1em}	
	\noindent\textbf{Multiple Identities to Multiple Identities (Many-to-Many).}
	
	\cite{zablotskaia2019dwnet}
	In this paper, the authors propose DwNet: a GAN-based architecture for single image body reenactment. The authors note that CNNs do not work well when the input and outputs are not well aligned. This means that motion information is needed to help the network translate a body to a very diffrent pose or position. To accomplish this, the authros propose a warp module which uses the target's pose (a UV map) to encode the target image warped to the source's pose (in the next frame). Using an ED network, the decoder is given (1) an encoding of the target's current pose, (2) the warp-encoding for the source image, and (3)  the warp-encoding for the last generated image. The pose is pobtained using a pretrained DensePose network [Densepose: Dense human pose estimation in the wild.] which outputs a UV map of the body segmented according to the limbs.
	
	[[note to reader that there are those papers which deatch the decoder at the outout (warp after through the sum dot map), and others which teach the warp motion at the input. Doing so at the input will require multiple frames at a time (ie video content), but will also result in smoothet content. Another approach to ensure the output video i smooth is to feed the last outputs back as inputs to give the decoder context as to wha tthe next motion should be. ]]
	
	
	The author propsoe a GAn for high resolution facial reenactment which works at extreme poses. Thier architecture consists of a face boundry transformer network and a face sythesis network. The boundry transformer network uses t(1) the encoder $En_{b1}$ encodes the target's boundry image $b_t$ to $v_t$, (2) two networks $P$ and $E$ estimate the pose vector $p_s$ and expression vector $e_s$ using the source's boundry image $b_s$, and (3) the concatenation of $e_s$, $p_s$, and $v_t$ are passed to the decoder $De_b$ which generates $b_g$, the boundry image of the target witht he source's expression and pose. To train this network, the authors use a combination of L1 loss on images with labeled expression vectors, and conditional regresson loss on randomly generated $e$ and $p$ on a given $v$ to cover unseen poses and expressions.
	
	%summarize and place in category by date (many-2-one...,date)
	\cite{zhou2019dance}
	\cite{siarohin2018deformable}
	\cite{balakrishnan2018synthesizing}
	\cite{de2019conditional}
	\cite{ma2018disentangled}
	\cite{zhu2019progressive}
	\cite{lee2019metapix}

==> sec_reenactment_uncut.tex <==

	[table: reenactment summary - general]
	
	[table: reenactment summary - training/datasets]
	
	[fig: reenactment schematics]
	
	%\subsection{Facial Reenactment}
	First we will review facial reenactment and then body reenactment
	
	\subsection{Expression Reenactment}
	
	
BEFORE DEEPFAKES

	\cite{blanz2003reanimating}
	The authors provide a facial reenactment system for single images using 3D scanning technology. The system (1) estiamtes the target's 3D shape and renderign parameters, (2) transfers the mouth movements and expression form the target's 3D facial scan, and (3) renders and blends the modified face back intot he image.	
	****not deep, pre deepfake and for still image animation, intro to reenactment of still image
	
	\cite{chang2005transferable}
	A paper on frontal facial reenactment usign a short sample video of the target (5 sec vs 10 minute of past stota). They accompliush this by matching the target's frames to the source's expressions, and by performing regression to fit the source's speech model to the target's. 
	***not deep, predeepfake. intro to reenactment becoimging easier
	
	
	\cite{thies2015real}
	In this apper the authors perform facial expression reenactment using an RGB-D camera and 3D head rendering. Their approach is to (1) capture the source and target's heads, (2) transfer the expression tot he target via model parameters, (3) accuratly  render the target's 3D face, and (4) blend the rendered face back into the target video. 	
	****not deep -pre deepfake?
	
	\cite{thies2016face2face}
	In this paper thauthors present an approach for real-time facial reenactment, that deos not use machine learning. At run time, the authors track facial expressions of both source and target video, and  reenactment is achieved though efficient deformation transfer between source and target face models. Finally, the best fitting mout interiror from the target is taken and warped before blending the face back into the target video.	
	***no ML, but core paper
	
	
	\cite{averbuch2017bringing}
	The authors propsoe a method for facial reenactment of portait images (no speaking) with confidence aware warping. The approach is to (1) extract the facial landmarks and superimpose a triagulation mesh over the image, (2) morph the image with the mech driven by a target's facial landmarks, (3) use a blur kernel to omit artifacts outside of the face, and (4) add hidden regions (inner mouth) and expression shading. 	
	***not deep, brings life or expression to image, to be cited very breifly in text
	
	\cite{thies2018headon}
	In this paper, the auhtors perform full facial reenactment with upper torso motion in a framework they call HeadOn. The approach uses an RGB-D camera to create a delegate mesh of the target and then drive the mesh with a source actor with pose-dependent texturing.	
	***Not deep, required RGB-D cam, but good example of how deepfake is not he only reeanctment tech
	
THE BEGINNING
	
	\cite{bao2017cvae}
	The authors propose CVAE-GAN, a generative network based on VAE-GAN where the generator is conditioned on an attribute vector or class label. The authros breify show how the networkm can be used for attrbute morphing (e.g.  pose), and otehr tasks sucha s inpainting.
	***good intro to other VAE and gans with fig

	
\noindent\textbf{Identity to Identity (One-to-One).}
	\cite{bansal2018recycle}
	The authors propose a generic translation network like pix2pix and cycleGAN called recycle-GAN. recyvcleGAN operates similar to cycleGAN except that it considers temproal aspects aswell by including next-frame predictor networks for both domains, and by introducing recycle loss. This apporach enables source agnostic video translation. For facial reenactment, the authors train their network to translate facial landmarks to talking portraits.
	
	\cite{liu2019video}
	The authors propose a framework for upperbody reenactment which can control a target's facial expressions, arms, and hands. For each source frame, the process is to (1) extract the facial AUs and pose as the vector $b_s$ and extract the upper body key points as the image $u_s$ using avalaible libraries, (2) normalize $u_s$ (denoted $u_g$) using the method in [everybody dance now] and use $b_s$ to generate the target's facial boundry image $b_g$ with a pix2pixHD GAN, (3) paste $b_g$ into the image $u_g$ to form $c_g$, (4) use another pix2pixHD GAN to generate $x_g$ from the concatenation of $c_g$ and the last $L$ generated images $x_{g}^{(t-1)},\dots x_{g}^{(t-L)}$. For temporal coherence, the authors employ a similar strategy as [everybodydancenow] by supplying the discerminator with $x_{g}^{(t)},\dots x_{g}^{(t-L)}$ and $c_{g}^{(t)},\dots c_{g}^{(t-L)}$. The last GAN is also trained with temporal smoothing, feature mathcing, and perceptual losses.
	***requires lots of source and target video footage
	
	\cite{tulyakov2018mocogan}
	In this paper the authors propose MoCoGAN: a temporal GAN which distangles motion and content (objects). The GAN recevies a random vector $z_c$ for the content and a sequence of random variables $[\epsilon^{(1)}, ...,\epsilon^{(K)}]$ which controls the motion.  The variables are passed through a reccurent nerual network to form the sequence of codes  $[z_{M}^{(1)}, ...,z_{M}^{(K)}]$. Next, a generator creates a video frame for each pair  $\{z_c,z_{M}^{(k)}\}$ in the sequence. Finally two discerminators are used to check the realism: one for image content and the other for the tempral cohernce of the last T frames. In their evaluation, the authors show how MoCoGAN can be used to perform both facial and body reenactment when trained with conditional variable (expression label) which replaces $z$. 
	***juxtapose with other gan that distangles motion fomr content
	
	
\noindent\textbf{Multiple Identities to a Single Identity (Many-to-One).}
	\cite{kim2018deep}
	In this paper, the authors perform complete facial reenactment by learnign from one minute of portriat video using a GAN. As opposed to previous works which reenact the expressions alone, here the authors transfer the full 3D head position including the expression (gaze, blinking, mouth, etc.). The apporach is to transfer the facial pose and expression from the attacker's 3D parametric model to the victim's, and then for each frame, pass the rendering information to a AE generator which creates a realistic output frame.  Each frame of the attacker's video is converted into the tuple consisting of (1) a rendered image of the victim's face on a black background using the attacker's pose and expression, (2) a correspondance map which is an image of the face where each vertex is colored with a unique color for tracking, and (3) a mask of the eyes and their gaze. The generator receives a sliding window of 11 converted frames where the output represents the last frame. To train the generator network, a GAN is used where the generator's input and target output (label) is taken from the victim's video footage alone. 	
	***good facial reenactment terms for taxonomy
	
	\cite{wu2018reenactgan}
	The authors propose a video-to-video facial reenactment method called ReenactGAN which transfers the expression of a driver's face to a target's face. Previous works have mapped the driver's pixels to targets face. In this work, the authors suggest that the input face should first be mapped to a `boundary latent space' (such as facial feauter bountries) which are identity agnostic to targets diffrent targets. To accomplish this, the authors use an ED network consisting of (1) a generic portrait to boundry encoder, (2) a target specific any-boundry to target-boundary transformer (converter), and (3) a target specific target-boundry to facial image decoder. The boundry transformer is a modified CycleGAN and the ED network is trained similar to a pix2pix network.	
	
	\cite{wang2018vid2vid}
	The author propsoe a video to video translation network. UNlike image-to-image translation networks like pix2pix, the rpopose network considers a spatio temproal adversrail objective to provide tempraol coherhnce and improve image quality. Conceretely, the generator predicts the next frame based on the current input and the last L inputs and generated images. The frameworks also uses two discerminators, one for per frame image quaility and the other for temporal coherehnce (optical flow for the last K consequitive frames). vid2vid uses a progessive traingin straegy on both the image resolutiona nd frame rate. The authors evaluate on a waide variety of tasks including face/body reenactment and attribute tampering.	
	***Not explicity facial reenactment (body yes) because input is face sketch, though easy to adapt to landmarks or other.

	
\noindent\textbf{Multiple Identities to Multiple Identities (Many-to-Many).}
	\cite{pham2018generative} 
	In this paper the authors present GATH: a facial reenactment GAN for animating a single target image with continuos action units (AU) as an input. In contrast to previsou works, GATH does not require a face model or image processing such as warping to drive a target portrait. The generator is ED network which (1) receives the source image as an input and (2) receives the target's AU vector internaly by concatentating it to the output of the decoder via spatial replication. The generated image is then passed to three networks: (1) an adversarail discerminator, (2) a face ID classifier, and (3) a pretrained AU estimator. The classifier shares the same hidden weights as the discerminator to help the generator distangle the identity from the expression. The AU estimator is used to signal the expression loss to the generator. The network also uses total variation loss to maintain smoothness.	
	
	
	\cite{shen2018faceid}
	The authors propose FaceID-GAN for full facial reenactment. Contrary to other works which use an identity classifier for perceptual loss, FaceID-GAN incoorperates the classifier within the adversrail game, competeing against the generator with the discerminator.  First $x_t$ is passed to an identity encoder $I$ and a face shape predictor $P$ producing $e_t$ and $p_t$, where $e_p$ is the face's 3DMM parameters. Next, a decoder $De$ produces $x_g$ using a concatentation of a noise vector $z$,  $e_t$, and $g(p_t)$ where $g$ is a function that transforms the pose and expression to that of $x_s$ usign a 3DMM expression. The model is trained using two discerminators: one for realism $D$ and the other is the same $I$ for identity. To minimize the supervison during training, $D$ is autoencoder discerminator (from BeGAN \cite{berthelot2017began}) which measures the resonctruction loss between a real and fake image. The discermiantor $I$ is trained as identity classifier for $N$ identites, where the first $N$ outputs are activated if the input is real and the following $N$ outputs are activated if fake. Finally, $De$ learns from $I$ and $D$ using adversarail loss, identity cosine loss, and learns from $P$ with L2 loss. In their evaluations, the authors show how FaceID-GAN produces high quality faces and at extreme poses.	
	
	\cite{shen2018facefeat}
	The authors in [shen2018faceid] then proposed FaceFeat-GAN which improves the diversty of the faces while preserving the identity.  
	Three encoder/predictor neural networks $P$, $Q$, and $I$, are trained on real images to extract feature vectors from portraits. $P$ predicts 3DMM parameters $p$, $Q$ encodes the image as $q$ capturing general facial features using feedback from $I$, and $I$ is an identity classifer which predicts the identity label $y_i$. Next two GANs, seeded with noise vectors $z_p$ and $z_q$, are trained to generate fake $p'$ and $q'$ feature vectors from the distributions of $P$ and $Q$ respectivly. Finally, a third GAN is trained to reconstruct $x_t$ from $(p,q,y_i)$ and $x_g$ from $(p',q',y_i)$ where the generator and discerminator consider recontruction loss on $x_t$, and the generator considers L2 loss on the identity using $I$. 
	To manipulate $x_t$, (1) the identity label $y_t$ is predicted using $I$ (even if the ID was not in the training set), (2) $z_p$ and $z_q$ are selected emperacally to fit $x_s$, and (3) the vector $(p',q',y_t)$ is used to generate the image using the final generator. The authors also note that additional semeatic features, other than those captured by $P$ and $Q$, can be added to FaceFeat-GAN."	
	***explains 3dmm face representation well, training does not require face pairs for supervised trainign of identities at diffrent poses
	
	\cite{nagano2018pagan}
	In this paper, the authors present a method for facial reenactment using a 3D avatar with single target image as input. The method is to (1) obtain an image of the victims's face (source) with a neutral expression, (2) use an existing algorithm to extract a 3D Model of the victim' face, (3) drive a target expression on the 3D model (e.g., from the attacker's captured face), (4) use a trained U-Net AE to generate realistic textures for the driven model using a masked image of the target with a neutral expression, a masked rendered face with the source expression, and the rendered face's UV map. The gaze is controlled by maskign the eyes in the rendered face and placing white points where the pupil should be (in painting).
	The AE which generates the realistic facial textures is trained using a GAN framework called pix2pix. 
	%Let....
	%I_s: an image of the source's face with a neutral expression
	%I_t: an image of the target's face with the target facial expression E
	%phi(M_E): a rendered image of the 3D mesh of I_s, driven with the expression E
	%delta(M_E): a depth map of M_E
	%gamma(I_t): a masked image of the eye gaze in I_t 
	%p(M_E,T_s): a rendered image of M_E using the texture from I_s (T_s)
	%The authors train the discerminator on tuples in the form of (I_s,phi(M_E),delta(M_E),gamma(I_t),p(M_E,T_s)) for fake samples, and replace p(M_E,T_s) with the Generator's output for fake samples. 
	The authors define the loss for their AE generator considering the pixel-wise loss and identiy preserving losss in aditional to adversarail loss. The identity preservin loss is obtained from a pretrained face identity model in [A light CNN for deep face representation with noisy labels.]]
	To make the process efficient for real-time deployment, the authors generate a large set of facial expressions offline for the victim (offline) and then blend the images accorinding to the drivivng expresion in real-time.
	
	\cite{sanchez2018triple}
	In this paper the authros propose GANnotation which uses a novel "triple consistency loss" for facial reenactment. Instead of just using self-consistencey loss like in [Ganimation], triple consistency loss imposes the generated image to reflect the target's distribution regardless of the number of translation steps used with consistnecey loss. In other words, it lets the network consider intermediate pose/expressions. The inputs tot he gnerator is the image concatenatied witht eh target landmarks where each landmark type spatialy fills a diffrent channel. Similar to [ganimation], their GAN uses an attention mechanism at the ourput of the generator to produce $x_g$. To train the model with triple consistency loss, the authors select three frames from the same video, over multiple videos of diffrent identities. 	
	
	\cite{wiles2018x2face}
	In this paper the authors propose a network called X2Face which performs full facial reenactment of a single portrait image using a driving video or other modality input (such as audio). The appraich is to use two ED networks: the embeddgin network and the driving network. The embedding network encodes 1-3 examples of the target's face to $v_t$: a 2D vector map with two channels (x and y) measuring the directional delta for each pixel required to transform $x_t$ to a neutral pose and expression. Next, $x_t$ is interpolated according to $m_t$ producing $x_{t}^{'}$. Finally, the driving network maps $x_s$ to the vector map $v_s$, crafted to interpolate $x_{t}^{'}$ to $x_g$, having the pose and expression in $x_s$. During training, first L1 loss is used between $x_t$ and $x_g$, and then an identity loss is used between $x_s$ and $x_g$ using a pretrained identity model trained on the VGG-Face Dataset. All interpolation is perfomed with a tensorflow interpolation layer to enable back propegation using $x_{t}^{'}$ and $x_g$. The authors also show how the embeddgin of driving network can be mapped to other modalities such as audio and pose.	
	***single iamge reeenactment
	

	\cite{yang2018pose}
	reeenactment. need summary
	
	
	\cite{tripathy2019icface}
	The authors present ICface: a facial reenactment method for single portriat images, where the expression and pose can be driven independantly. Their architecture is similar to a CycleGAN with some modifications: During training, a source and target image is taken from the same video. The first generator is used to convert the source image to a neutral expresion and the second generator takes the generated neutral image and converts it to the driving image, where both generators use the same discerminator. To condition the facial expressions, the generators are supplied with the target facial attributes: a $R^20$ vector with the pose direction and expression levels (a.k.a. action units or AU). The facial attribute vector is merged with the input image by (1) encoding the image to with a CNN, and (2) adding the 20 attributes as additonal channels to the encoded image (spatially filling each channel). In their evalution the authors showed how they can drive a target's expression, pose, mouth, eye, and eyebrows seperetly from a source image.
	

	
	\cite{zhang2019faceswapnet}
	An issue with landmark based facial generation is that the shape of the sources face leaks through to the generated image [[cite landmark based paper that notes this]]. In this paper the authors circumvent this issue with FaceSwapNet which is agnostic to a target's shape and pose. First two encoders and a decoder are used to transfer the expression in $l_s$ to the face structure of $l_t$, denoted $l_g$. Then a generator network is used to convert $x_t$ to $x_g$ where $l_g$ is injected into the network with AdaIn layers like a Style-GAN [https://arxiv.org/pdf/1812.04948.pdf]. To adapt this type of generator to their task, the authors found that it is crutial to use triplet perceptual loss (using the VGG network) in additon to the adversarial and L1 loss. In their evaluation, the authors were able to generate high quality portriats driven with various expressions and at diffrent poses.
	***they use HyperLandmak to fins facial landmarks,very good quality
	
	
	\cite{pumarola2019ganimation}
	In this paper the authors propsoe a facial reenactment (expression) method called GANimation which produces anatomicaly consistant animations with a custom GAN architecture. Given an image, the trained model can gradualy adjust any of the faces expression attributes called action units (AU). Their architecture uses (1) a generator which utilizes a self attention model to transform a face according to a given AU vector, (2) a WGAN-GP inspired discerminator is used to evalaute the iamge quality, and (3) another network, with some shared weights with the discerminator, is used to penalize errors in the generated expression. Similar to the cycleGAN image translation network, during training GANimation passes an output back through the generator again to reverse the manipualtion and mesuare the cycle consistnecey loss. As a result, GANimation is train in a fully unsupervised manner where no image pairn is needed. Moreover, the authors note that the attention model enables the generator to handel images with distracting backgrounds, illumination artifacts, and occulsions.	
	
	\cite{nirkin2019fsgan}
	In this apper the authors present FSGAN: a face swapping and facial reenactment model. Thier approach is
	subject agnostic, meaning that is can be applied to any pairs of faces without requiring training of the model, and can work on a single image of the target. Furthermore, FSGAN succeeds at in cases where the target face is partially covered or unseen (such as hair over the face or the inside of the mouth). Their apporach is also efficent achieving 30fps for facial reenactment and 10fps for face replacement. 
	
	To accomplish this, FSGAN uses four AEs trained in GANs: $G_r, G_s, G_c$, and $G_b$ where $G_r$ is needed for facial reenactment and all of the NNs are needed for face replacement:
	
	The recurrent reenactment generator $G_r$: The purpose of $G_r$ is to reenact a target image $I_t$ with a given source image $I_s$. The input is the source image $I_s$ and the target expression $p_i$, represented as 2D image of the target's face landmarks using 70 channels (one for each landmark ID). The output is a reenacted face image $I_r$ and its segmentation map $S_r$ with three channels (background, face, and hair). The generator $G_r$ is trained recurrently where each output is passed back as input for several iterations while $p_i$ is interpolated incrementally ($p_{i+1},...$) between the source's and target's facial landmarks. For a seemless reenactment, the authors suggest selecting a source image (e.g., from a sample video) with a face position similar to the target's. To accomplish this, the authors query images of the source with Delaunay Triangulation and generate a new image with barycentric coordinate interpolation. $G_r$ is trained on videos of many diffrent individuals with a perceptual, reconstruction, and adversarial loss.
	
	The segmentation generator $G_s$: The purpose of $G_s$ is to find a segmentation map $S_t$ for the target image $I_t$. This is needed to identify the areas on the reenacted face $I_r$ which are missing an need to be recontructed using inpainting. $G_s$ is trained inturn with $G_r$ and uses cross entropy loss as well as recontruction loss between the predicted map and the map from $G_r$.
	
	The inpainting generator $G_c$: This generator performs inpainting on the reenacted face in $I_r$ so that missing areas are recontructed accuratly. The masks $S_t$ and $S_r$ are used to identify the missing pixels in $I_r$ needed to fit the face in $I_t$. Given the inpainting mask and the face in $I_r$, $G_c$ completes the missing pixels to create the face $F_c$. The model is trained by randomly removing elipses from images of faces with an adversarial and recontruction loss. 
	
	The blending generator $G_b$: This model blends the completed face $F_c$ into the target image $I_t$ while considering ethnicity and lighting. The model receives $I_t, I_{t}^{r}$, and $S_t$ where $I_{t}^{r}$  is $F_c$ pasted onto $I_t$, and outputs the final face replacement image. The model is trained using a combination of Piosson optimization and perceptual loss, and adversarail loss.
	
	With the exception of $G_s$, the NNs followed pix2pixHD architectures using coarseto-fine generators and multi-scale discriminators.
	***juztapose with reeactGAn on agnostic subject for reeenactmant. Build up:
	37, 50, 40, 11, These methods decompose the identity
	%component of the face from the remaining traits, and encode identity as the manifestation of latent feature vectors,
	%resulting in significant information loss and limiting the
	%quality of the synthesized images 45, 34, 33
	%Subject specific methods [42, 11, 50, 21] must be trained for each subject or pair
	%of subjects and so require expensive subject specific data"
	
	\cite{qian2019make}
	In this apper the authors propose Additive Focal Variational Auto-encoder (AF-VAE) for high quality facial reenactment that is both diverse and identity agnostic. This is accomplished by seperating a C-VAE's latent code into an apperance encoding $e_a$ and identity-agnostic expression coding $e_x$. Further more, to capture a wide vareity of factors in $e_a$ (e.g., age, illumination, complexion, ...), the authors (1) us K-means to cluster the facial bountries in their dataset into clusters, and (2) model $e_a$ as a Gaussain Mixture where each Gaussain kernel is represented by the mean and standard deviation of each cluster accordingly. The authors refer to this process as an novel additive memory module and is used only during training. Overall, the architecture is as follows: One encoder uses $b_s$ to encode $a_e$ and another encoder uses the concatenation of $b_s$ and $x_t$ to encode $e_x$. Finally, $e_a$ and $e_x$ are concatenated and paseed through a decoder to produce $x_g$. In the decoder, the authros use subpixel convolutions to removel artifacts and improve fidelity, and skip connections with the structure encoder to preserve identity. To increase the diversity of the generated images, the authros train the model using  weight normalization. Furthermore, the authors propose a human inception score which can be used in user studies to rate the fidelity of a generatel face and demontrate their method on the task of hand reenactment.
	
	
	
	\cite{zhang2019one}
	The authors propose a facial reenactment system which also controls gaze. They (1) use a network to produce a multi-channel segmenation of the source's face, (2) encode the apperance of the target with an encoder, and then (3) produce $x_g$ with a decoder that receives the target's encoding as an input and the source's segmentation at inner layers using SPADE residual blocks. Finally, to mitigate artifacts in the background and speed up convergence the authors blend $x_g$ with a warped version, guided by their facial segmenation masks.
	
	

	
	\cite{fu2019high}
	The face sythesis network is a GAN consisting of two encoders and one decoder. The first encoder $En_t$ encodes the face textures of $x_t$ as $t_t$. The second encoder $En_b2$ encodes the transformed boundry image $b_g$ as $v_g$. Finally, a decoder $De_g$ receives the concatenation of $t_t$ and $v_g$ and generates $x_g$. During training, a pretrained face recognition network is used to extract an encodign of the target's face structure. This encodign is used to distangle the $En_t$'s outputs from the facial structure using a novel threshold feature loss. The authors also use featuremating loss, a multi-scale L1 loss, and and three conditional discerminators at diffrent image scales. In their evalaution the authros show how their method works well at high resoltuiosn and at oblique angles.
	%The dataset they created is of HiRes images of actor head taken at several diffrent angles.
	***Nice method for semisupervised learnign of expression transformation using a small labeld dataset as a start  (then random gen seeds passed through decoder and validated on the predictors)"
	
	\cite{MarioNETte:AAAI2020}
	The authors propose MarioNETte: a few-shot facial reenactment network that preserves the identity of targets unseen during training. The authors note that other techniques leak the driver's identity into the source or gnereate artifacts when the target pose is very diffrent than the source's.To transfer the identity of target to a source driver, previous works would either encode the target's identity and concatenate it with an expresssion vector or insert it with AdaIN layers (e.g, [zakharov2019few]). However, these approaches result in a loss of spatial information of the target.  To preserve the target's identity, the authors use an image attention block and target feature alignment. The attention block is similar to the ED attention transformer of \cite{vaswani2017attention} where the source's feature map is used to query the target's feature map, thus preserving the spatial information. To preserve the target's identity, the authors also use target feature alignment which warps the target's low-level featuremaps.This enables the model to better handle the diffrneces in the face structures. This is done by creating a pose normalized featuremap of the target's feature maps and then by aligning them to the pose of the source. Furthermore the identity is preserved using a novel landmark transformer. Inspired by [A morphable model for the synthesis of 3d faces], the transformer decomposes portrait into expression and identity geometries using landmark normalization and a neural network. Then a new landmark image is created by replacing the target's expression geometry with the source's.
	
	Overall, the proposed network works as follows: given $x_s$ and $K$ samples of the target $x_{t}^(K)$, (1) the landmarks of $x_s$ are extracted and passed through an encoder $En_s$ to extract the driving pose and expression as $e_s$, (2) the landmark transformer produces the landmark images $l_{t}^(K)$ from $x_{t}^(K)$ with the expression of $x_s$, (3) . The pairs $(l_{t}^(i),x_{t}^(i))$ are passed though the encoder $En_t$ to produce featuremaps $v_{t}^(i)$ and warped feature maps $w_{t}^(i)$, (4) an image attention block blends $e_s$ and $v_{t}^(i)$ together producing $e_{st}$, and (5) the decoder $De$ uses $e_{st}$ to generate $x_g$ with feature alignment using  $w_{t}^(i)$ on the inner layers. 
	
	
	
	\cite{geng2019warp}
	A well-known approach for facial reenactment of single iamge portriats is to warp the target image usign facial landmarks mapped to a driving actor's face [elor2017bringingPortraits]. In this paper, the authors propose wgGAN which uses the same approach but creates high-fidelity facial expressions by refinign the image with two GANs. The appraoch is to (1) find the facial landmarks of the driving face and target face, (2) warp the target face according to the driving face's landmarks, (3) pass the masked warped face and its normalized pixel displacement (vector) map to a GAN which improves the quality of the warped image, and (4) pass the refined masked face to another GAN which performs inpainting on the mouth region. The generator is trained in in a GAN using public video datasets, where a rest expression frame is used as the target and every 10th frame is used as the driving expression.
	A challenge with wgGAn si that the warping process is sensitive to head motion (change in pose).
	***single iamge reeenactment

	
	\cite{siarohin2019animating}
	The authors propose Monkey-Net: a self supervised network for generating video where an image of a target object is animated according to a driving video sequence. Similar ro MoCoGAN [], the authors decouple the source's content and motion to drive arbitrary content (still iamges). First a task specific key-point detector is used to extract keypoints from the current source frame and the target image. Next, the keypoint changes and the target image are passed to a dense NN which predicts the motion heat map (optical flow) necesary to drive the target object from its current state to the source's. Finally, a ED generator receives the target image as an input, driven by the keypoint changes and the motion heatmap which are inserted into decoder's inner layers. The authors evalaute their network on the task of facial reenactment and body reenactment.
	
	\cite{otberdout2019dynamic}
	"In this paper, the authors propose Motion \& Texture GAN for smoother facial reenactments of neutral expression faces. Similar to [MocoGAN], the authors use a two step process which processes the motion and content sythesis seperatly. The authors state that animations of facial landmarks, between the neutral expression and a target expression, can be described as temporal curves in 2D space. These curves can be sumamrized as points on a spherical manifold by calculating its square-root velocity function (SRVF). Knowning this, the authors aim to generate points (on a tangent on hypersphere) using an WGAN given a random noise vector and a target expression label. Once the SRVF point has been generated, the authors apply the SRVF to the target's neutral expression landmarks which generates sequence of facial landmarks witht he target's facial structure.  Finally, a pix2pix GAN is used to convert the sequence into a video of the target.
	**Note to reader that some methods smooth provide temporal coherence by feeding the video to a D, others do so by crafting the input frames carefuly before texture generation (like this one)
	
	\cite{NIPS2019_8935}
	The authors extend their work on Monkey-Net \cite{siarohin2019animating} by improving the object appearance when large pose transformations occur. They accomplish this by (1) modeling motion around the keypoints using affine transofmations, (2) updating the keypoint loss function accoridly, and (3) having the motion generator predict an occlusion mask on the preceding frame for inpainting inference.
	***juxtapose right after Monkey-Net
	
	
	\cite{wang2020imaginator}
	[paper animates face with label as transition, no explicit deep fake application]
	In contrast to MoCoGAN, the authors of this paper propsoe a conditional GAN which fuses both motion and content, but with transposed 3D convolutions to capture the distinct spatio-temporal relationships. First a CNN encoder compresses the input image into a spatial feature vector. Next, the encoding is concatented with a label (e.g., emotion or expression label) and a random vector. Finally, the vector is passed through the decoder network which produces a set of video frames. The decoder neworks uses blocks which perform 3D convolutions over a concatenation of the spatial and temproal feature maps with U-Net like skip connections from the decoder to utilize the input image for spatail refrencing. The GAN uses a image and video (temporal) discerminator, where the temporal discermiantor uses similar 3D convolution blocks as the decoder and receives the label as context. To increase diversity, the authors also train the video discerminator with some videos using the wrong label.
	***Some downsides are that it is label driven and that the output has a static length in video frames.
	
	
\noindent\textbf{Few-Shot Learning.}

	\cite{zakharov2019few}
	The authors propose a full facial reenactment method which requiring only one or more images of the target. Their method preserved the target's identy at a wide range of facial poases unseen in the training data. To accomplish this, the authors utilize a method in deep learing called few-shot learning  [https://arxiv.org/pdf/1812.02391v3.pdf], expanded from one-shot learning []. The approach is to (1) pretrain (meta-learning) on a large dataset of talking portiat videos by learning to transform facial landmarks to realistic images given only a few examples of each identiy, and then (2) perform adversarial traingin on a few images of the target for just a few training steps. During meta-leraing, three networks are trained in a GAN setup as follows: For each identity, (1) an emedder network takes a few images of the individual, contatenated with the facial landmarks, and converts them into embeddgins which are averaged into a single identity embedding $e_i$, (2) an AE generator network takes the landmarks of a diffrent image of the identity, and converts it back to the image, where $e_i$ is used internally adaptive isntace normalization (AdaIN), and (3) a discerminator validates the ralsim of the generated image given the facial landmarks using a match loss. The discerminator also receives as an input a one-hot encoding of the video clip from which the frame was taken from, and a hinge loss is applied to $D$ to ensure consistencey. Finally, the network is tunned to a new target by passing one or more images through the encoder, and training the updating the parametes of the model accoridngly. As future work the authors aim toa ddress the sensativity which the driving face has on the appearance of the target's generated face.
	***add example frame from video
	
	\cite{wang2019fewshotvid2vid}
	In this paper propseo a few-shot vid2vid framework by expanding their origional vid2vid framework with a network weight generation module that utilizes an attention mechanism. The module learns to extract appearance patterns which can be injected into the video synthesis layers. The authors evalaute their frame work on single image reenactments of faces and bodies, among other tasks.
	***advances video-to-video by reenacting single images
	
	
	\subsection{Mouth Reenactment (Dubbing)}
	Lite intro
	
		
	\noindent\textbf{Multiple Identities to a Single Identity (Many-to-One).}
		\cite{suwajanakorn2017synthesizing}
	In this paper, the authors create a realistic reenactment former president Obama by replacing his mouth with new video content generated from an audio input. Using a large dataset of Obama's weekly addreses, the authors accomplish this with three stage process: take a target video of a Obama giving a speech, then (A) map the input audio segments to observed mouth shapes, (B) generate mouth textures from mouth shapes, and then (C) blend in the generated mouth area into the target video clip and retime video so the head motions match the input speech. 
	For mapping audio to mouth shape the approach was to (1) extract a 28 dimensional feature vector for each 25ms segment of audio containing 13 MFCC coeffeicnst, volume, and tempral derivaive features, (2) for each audio segment, extract the mouth shape as a 36 dimensional vector using landmark detection and use PCA to reduce the vectors to 20 dimensions, and then (3) map audio segments to mouth shapes using a time delayed RNN (delayed to cosider the next utterance as well). 
	For mapping mouth shapes to mouth textures (cropped mouth and bottom nose area), the authors performed the following: (1) for each PCA mouth shape find a fixed number of target video frames that best match it, (2) apply weighted median on the frames to create the representative texture, and (3) refine the teeth in the texture by selecting similar frames from the target video and transfering the high-frequency teeth
	details into the texture.
	Finally before blending the texture into the target video, dynamic programming is used to speed up and slow down the target video so that more head motion is associated with speech and vice versa.
	
		\cite{jalalifar2018speech}
	The authors propseo a video dubbing system that geenrated video based on audio alone. Unlike [lip sync obama], the output is fully sythesized and thus no frame timing is needed to match the head pose. Their system has two parts. The first part uses a bidirectional LSTM to translate 33ms clips of source audio (MFCC features) into a sequence of mouth landmarks. The second part uses a GAN that takes a noise vector concatenated with the landmarks and produces a sequence of frames. Similar to pix2pix, the D receives a real/fake image and the condition (the landmarks). Since their lip modeling network is trained seprate from the image generator, the system works well using udsio from diffrent poeple. After trainign the generator on many videos of the target, the network is fine tuned using a single video of the target to ensure consistent textures and background.	
	
		
	\cite{fried2019text}
	In this paper the authors propose a method for editing a transcript of a talking head which modified the target's mouth and speech according to the edited text. With this technology, and attacker could change the meaning of a speech by changing a few words or even rewrite it entirely. The approach is to first align phenomes to the input audio track, and create a 3D parametric head model tracked to each input frame. Then, for each edit operation on the transcript, (1) new words are created by blending matching phenomes found in a corpus of the target's speech, and (2) the mouth is animated by blending the parametric 3D model states taken from the respective frames. Finally, a photorealistic mouth animation is created using an RNN which maps a synthetic composite (rendered mouth placed over the origional face) to an origial frame. The RNN architecture was inspired by [High-Resolution Image Synthesis and Semantic Manipulation with Conditional GANs]. It is trained three frames at a time using a GAN with a spatial discerminator and temporal discerminator. To imrove the quality of the mouth region, the authors use a loss function which focuses on errors in the mouth region using a Hadamard product. In the end, the quality of the mouth is improved compaed to the work of [face2face] [[[screen shot image from demo video]]].
	***The 3d modeling approach is from ""deep video portraits""
	***one model per target
	
	\cite{kumar2017obamanet} text to obama, NN
		
	\cite{thies2019deferred}
	The authors introduce Deferred Neural Rendering for image synthesis. The system can render realsitic imagery given basic rendering components of a 3D scene (e.g., uv-maps and textures) in a format referd to as neural textures. The neural textures are then used by a neural renderer (a modified U-Net) to dynamically render images of the scence from various viewpoints. In 
	\cite{thies2019neural}
	the authors use this technique to perform video dubbing which they call neural voice puppetry. Their system receives a voice and dubs a target's portriat video accordingly. To process audio, a sliding window of 300ms in strides of 20ms is passed over and audio clip. The system has two components: a target generic component that translates audio to vector representations, and a target specific components trasined to convert these vectors to 3D face blendshape parameters which then used as an input to a neural rendering network that generates the manipulated face, based on their preivous work in [thies2019deferred].  In the target generic component, the vecots are gnerated by (1) passing the window of audio to a pretraiend DeepSpeech [] model, (2) extracting the vocal expression matrix, and (3) generate $x_g$ by passing the matrix through a CNN that uses temporal content-aware filtering for temporal coherence. In the target specific component, the neural renderer uses two networks: one that renders a neural texture of the lower face created from a 3D rendering, and anotehr that blends the neural texture into the origional frame. The authors found that the target specific component only requires 2-3 minutes of video for training ont he target's speech expressions. 
	
	
			
	\noindent\textbf{Multiple Identities to a Multiple Identities (Many-to-Many).}
	\cite{liu2011realistic}
	In this apper the authors perform video dubing with the smilign expression for facial reenactment. The target is recorded in a studio reading text with neutral and smiling expressions. Then the animated talking head is rendered by parsing new text/audio (from TTS) and matching it to the most approapraite mouth region in the corpus.
	**not deep

	\cite{zhou2019talking}
	The authors propsoe a single image voice dubbing framework which involves a shared speech latent space for audio-based and video-based (mouth movement) content, and a latent space for a video-based visual identity. Their approach is to learn the speech latent space from short video clips containing words, while distangling the embeddings from the identity space, and then (2) combine the embeddings from both spaces together as an input to a GAN which animates the source's head. The generator takes an identity encoding and a speech encodign to produce a dubbed video. For temporal coherence, the GAN uses a temporal discerminator that considers a sequence of frames. Since either video or audio can be encoded into the speech space,  the user can choose on whether to dub an image based video (mouth movement) or audio. Furthermore, since the speech is distangled from the source's identity, the generator is target agnostic.
	
	\cite{jamaludin2019you}
	In this paper the authors propose Speech2Vid: a realtime video dubbing network that can operate on unseen images and audio during training. Their framework is also trained in a self supervised manner meaning that only video clips are needed without sematics, manual paring, or labeling. The architecture consists of two encoders (audio and identity) and a decoder which generates the video frame. To generated video, a window of 350ms slides over a source audio clip with a stride of 40ms. Each audio segment is sampled at 100Hz and converted into 12 MFCC features resulting in a $12x35$ feature map. The feature map is then passed through the audio encoder based on VGG-M which produces the encoding $e_a$. Next, the face region from five images of the target are sampled under similar lighting conditions, concatenated channelwise, and passed to the identity encoder producing $e_i$. Next, $x_g$ is created by passing the concatentation of $e_a$ and $e_i$ to the decoder which is a reverse VGG-M model with skip connections from the identity encoder to preserve the target identity. Since $x_g$ is blurry from the L1 loss used by the decoder, the authors sharpen the image using a VDSR CNN [Accurate image superresolution using very deep convolutional network]. This network is trained seperatly to reconstruct images which where artificailly blurred. Finally, the mouth region is blended into the target video with alignment and poisson editing. The authors also suggest an improved blending by adding a third context encoder, similar to the identity encoder, but with the mouth masked for the task of inpainting.
	
	During training,  the model uses a video's audio as the source, and five frames from the current window as the identity, and the center frame as the supervised output for $x_g$. To prevent lighting artifacts throughout the video, the authors use content represeantion loss with a pretrained CNN. Content loss is the weighted L1 loss between the actiavtions of a pretrained CNN [Photographic image synthesis with cascaded refinement networks]. 
	

	\cite{vougioukas2019end}
	In this paper, the authors propose a GAN-based system for audio driven video dubbing of a single target image, without relying on handcrafted intermediate features. Their system also affects facial expressions such as eyebrow moments and eye blinking. The authors perform a user study and found that the temporal GANs produce more realistic videos than static ones. The generator receives a single image and 160ms of overlapping audio, and consists of (1) a CNN which encodes the image's identity, (2) a CNN audio encoder connected to a two-layer RNN (GRU) for encoding the context, (4) a GRU based temporal noise genrator, and (3) a stride transposed CNN decoder which generates video frames with the concatenatination of the identy, context, and noise vectors. The identity encoder and the decoder follow the U-Net architecture with skip connections to preserve the target's identity. The framework uses two discirminators: one for image quality and the other for temporal coherence. The temporal discerminator uses two RNN encoders (for the current video frame and audio segment) whose encodings are passed to a 2 layer classifier. When applying the L1 loss, thne authors focus on the lower half of the face to encourage better lip sync quality over facial expressions.	
	***juxtapose just before their other work that expands it (noted above..)
	
	\cite{vougioukas2019realistic}
	In this paper the authors expand their work from [vougioukas2019end]. As opposed to other works which focus ont he mouth region only, this work also generates natural blinks and expressions in sync with the source audio. They accomplish this by splitting their temporal discerminator into two: (1) for temporal realism in mouth to audio sychronization, and (2) for temporal realism in overall facial expressions. By isolating expressions from synchronisation, the authors further encourage the generator to produce spontaneous facial expressions, such as blinks. They also provide a temporal noise signal for the generator to produce the dynamic facial expressions. [[detail what is left out (the dif) with my description of the other paper]]
	***Limitation: frontal only!!
	%....**copied from their next paper about this paper***: 
	%The identity encoder takes as input a single face image
	%and passes it through a 6-layer CNN, where each layer has
	%strided 2D convolutions, batch normalization and ReLU activation functions. The audio encoder receives a 0.2s audio
	%signal and passes it through a network of 1D convolutions
	%with batch normalization and ReLU activation functions, followed by a 1-layer GRU. The noise encoder receives a gaussian noise input which is passed through a 1-layer GRU. The
	%purpose of the noise encoder is to introduce some natural
	%variability in the face generation such as blinks and eyebrow
	%movements
	%the three encodings which is then fed into the U-Net
	%based [10] generator, along with skip connections from the intermediate layers of the identity encoder, to produce a frame
	%from a video sequence"
	***great relworkd on video dubbing via deep, juxtapose after their other work: End-to-End Speech-Driven Facial Animation with Temporal GANs
	
	
	\cite{kefalas2019speech}
	Later in this paper, the authros improve the work of [vougioukas2019realistic] by fusing the encodings (audio, identity, and noise) with polynomial fusion layer as oppesed to simply concatenating the encodigns together.  With concatention, the represetnation becomes sensative to large facail motions [Attention guided deep audio-face fusion for efficient speaker naming]. Instead, their approach enables the network to account for higher-order interactions and prevent the statistical domination of a subset of the represeantitions. The authros provide several methods of polynomial fusion and compare their work to [Speech2Vid] and [vougioukas2019realistic].	
	

	
	\cite{chen2019hierarchical}
	The authors state that direct models are problematic since the model learns irrelivant correlations between the audiovisual signal and the speech content. To avoid this issue, the authors first learn a direct mapping from audio to facial landmarks, and then model the mapping from the landmarks to the target identity. The audio-to-landmark network is an LSTM which receives the audio MFCC features and a compressed PCA representation of the coressponding facial landmarks.
	% The LSTM outputs the corresponding seqeunce of predicted compressed facial landmarks which are then expanded to full facial landmarks. 
	The landmark-to-identity network uses a convolutional RNN (CRNN) to generate the target's images using the sequnce of generated landmarks and latent information about the target's face. The authors adapt the attention mechanism from [Ganimation] by disentangling the motion from the audiovisual-non-correlated regions. Doing so help generate static pixels in regions that are not correlated to audio, and vice versa.
	To mitigate jitter, the authors introduce a dynamic pixel-wise loss with an attention mechanism. In additon, to improve face synchronization, the authors propose a regression based discermiantor which considers both sequence and content information. 
	
	\cite{nakashima2020speech}
	The authors perform video dubbing where the source and target are the same person... mostly uses cgi. Not so mal oriented bc requires source to look and sound the same.
	
	%summarize and place in category by date (many-2-one,date)
	\cite{shimba2015talking} Needs summary, NN

	
	\cite{song2018talking}
	\cite{liu2020synthesizing}
	\cite{yu2019mining}

	
	\subsection{Pose Reenactment}
	\cite{hu2018pose}
	note: facial reenactment of pose alone has mostly been researched for the task of frontalization [][][]. Some works have researched pose driven manipualtion, usch as ....
	They use a U-Net to convert a concatenation of $x_t$, $l_t$, and $l_s$ into $x_g$ using two discerminators. One discerminator distinguashed between real/fake rotated heads given the real head at a neutral pose, and the other discerminator distiguishes between real/fake heads at the same pose, given their landmarks.
	***to be cited very breifly in text
	
	\cite{tran2018representation}
	The authors propsoe DR-GAN for facial reenactment of pose for the task of pose-invariant face recognition. To adjust the pose of $x_t$, the authors use an ED GAN which encodes $x_t$ as $e_t$, and then decodes $(e_t,p_s,z)$ as $x_g$, where $p_s$ is the sources pose vector and $z$ is a noise vector. The authors show that the quality of $x_g$ can be improves by averaging multiple examples of $e_t$ togetehr before passing it through the decoder.	***to be cited very breifly in text
	
	\cite{cao20193d}
	The auhtors propose a system of two GANS for facial pose reenactment. The first GAN convert the face $x_t$ to a frontalized face image $x_{t}^{(f)}$ and its UV corrispondance map $uv_{t}^{(f)}$. This Gan is trained though adversarail loss on real/fake frontalized portraits and the UV map recontruction loss based on a 3DMM model extraction of the face for the ground truth. Next the second GAN utilized an ED generator to converts $(x_{t}^{(f)},uv_{t}^{(f)})$ to $x_g$, where the encoding is concatenated with the source's angle before going through the decoder.
	***to be cited very breifly in text
	

	
	\subsection{Gaze Reenactment}
	Some works have looked into facial reenactment of only gaze [][][] for the purpose of touching up images. For example,...
	
	\cite{ganin2016deepwarp}
	The authors peform gaze reenactment. The authors convert a cropped eye $x_t$, its landmarks, and the source angle, to a flow (vector) field using a 2-scale CNN. The flow field is then applied to $x_t$ warp it to the source angle, resulting in $x_g$. The auhtors then correct the illumination of $x_g$ with a second CNN.
	
	\cite{kononenko2017photorealistic}
	
	\cite{yu2019improving}
	The authors propose the Gaze Redireciton Network (GRN) for gaze reenactment using an ED network with cycle consistency loss. First the target's cropped eye $x_t$ is encoded and concatentated with target's head pose encoding and the source gaze angle encoding. Then the decoder produces a warp feild which is applied to $x_t$ to produce $x_g$. To overcome the lack of training data and the challenge of sample pairing, the authors (1) pretrain their network on 3D sythesized examples, (2) further tune their network on real images, and then (3) fine tune their network on 3-10 examplesof the target."
	***to be cited very breifly in text
	
	\subsection{Body Reenactment}

	==== mentioed in expression section, can be used for body too: ===
	\cite{wang2018vid2vid}
	\cite{wang2019fewshotvid2vid}
	\cite{tulyakov2018mocogan}
	\cite{siarohin2019animating}
	\cite{NIPS2019_8935}
	
		
	\noindent\textbf{Multiple Identities to a Single Identity (Many-to-One).}
	
	\cite{liu2019neural}
	In this paper the authors perform body reenactment and try to overcome some of the artifacts which occur in [everybody dance now] such as in correct detectio of skeletons which leads to stretched limbds. In their approach, the authors first build a 3D character model of their target with photogrammetry software and then animate it with the source actor's motion capture [MonoPerfCap: Human Performance Capture from Monocular Video]. The rendered model is then used to generate a realistic body on a given background using a pix2pix model. The input to the generator is the rendered body and their depth maps partitioned, and the target background. The discerminator uses applies L1 attention between $x_g$ anf $x_t$ on the adversrail loss to help the generator focus on relivant details as opposed to elemetns such as the static background. Approximalty 12k frames are used to train new generator per target with the pix2pix network. A challenge is that the attacker would need to obtain 100 images of the target from multiple angles with the same open pose in order to generate the 3D mesh character.	
	

	
	\cite{aberman2019deep}
	In [everybidy dnce], the authors train on paired data [[[[check]]]] which does not generalize well to unseen poses leading to artifacts. In a concurrent work to [everybody dance now], the authors in this paper mitigate this issue by using an upaired training branch with many identities other than $s$ and $t$. This also result in a reduction of training data from result 20min to 2min. Their model is a DNN which takes a 3D pose \cite{cao2017realtime} as an input and generates an image of the target's body in the given pose. To train their DNN, they use a GAN with two discermiantors over two training stages. In the first stage, the generator is trained on pairs of the target's pose and orgional frame using a combined loss from a discerminator. The discerminator considers whether a pose is real or fake given the frame, and whether the generated image is real or fake based on the the pose. The loss from a pretrained VGG-19 network is included to improve texture quality. After a few epochs, the loss function is extended by adding the loss of another discerminator which considers temporal coherence to ensure that the generator can translate unseen poses. The additional loss includes (1) the error between the current generated frame and the previouly gneerated frame after warping the previously generated frame with an optical flow field, and (2) the discermiantor's adversarial loss on predicting whether or not the pose is real or not (uncoupled to the input frame). The GAn was trained using 3000 video frames taken from the target performign various activitities. 
	
	\cite{chan2019everybody}
	The authors propsoe a mehtod for body reeanctment (dance) using a pix2pix GAN archotecture with a custom loss function. To capture the actor's pose for the network to intrepet, the authors convert frames into stick figures by (1) usesing an existing pose detector to extract the 2D x, y joint coordinates, and then (2) using the coordinates to plot key points and limbs as colored lines. The authors then train their GAN where the generator receives the curent pose and generates the frame, and the discerminator (1) verifies the realsim of the imagery conditioned on the pose, and (2) verifies temporal coherehence of the current and last generated frames conditioned on the pose. The authors also include the loss objectives from pix2pixHD and a pretrained VGGNet to improve texture quality. After training the generator, the weights are frozen and an additional pix2pix GAN is trained on the face region alone to improve the realism of the face. The face GAN is trained on a concatentation a cropped face (generated / real) and the respective cropped stick figure, where the generator receives concatentions of fake images only and produces the residual image that is used to imrove the generated image. The GAN is trained on 8-30 minutes of video footage on the target performign acticitities (dancing). To use the trained generator, the process for each frame is to (1) extract the driver's pose, (2) normalize the pose to the target's body, (3) pass the normalized pose through the body generator, and (4) improve the face region by passing the face through the face GAN. 
	***The authors also propose a method for detecting fake videos. They train a detector based on two consequtive frames which is trained in parralel to their GAN's sythesis process.
	
		
	\noindent\textbf{Multiple Identities to Multiple Identities (Many-to-Many).}
	
	\cite{zablotskaia2019dwnet}
	In this paper, the authors propose DwNet: a GAN-based architecture for single image body reenactment. The authors note that CNNs do not work well when the input and outputs are not well aligned. This means that motion information is needed to help the network translate a body to a very diffrent pose or position. To accomplish this, the authros propose a warp module which uses the target's pose (a UV map) to encode the target image warped to the source's pose (in the next frame). Using an ED network, the decoder is given (1) an encoding of the target's current pose, (2) the warp-encoding for the source image, and (3)  the warp-encoding for the last generated image. The pose is pobtained using a pretrained DensePose network [Densepose: Dense human pose estimation in the wild.] which outputs a UV map of the body segmented according to the limbs.
	
	[[note to reader that there are those papers which deatch the decoder at the outout (warp after through the sum dot map), and others which teach the warp motion at the input. Doing so at the input will require multiple frames at a time (ie video content), but will also result in smoothet content. Another approach to ensure the output video i smooth is to feed the last outputs back as inputs to give the decoder context as to wha tthe next motion should be. ]]
	
	
	The author propsoe a GAn for high resolution facial reenactment which works at extreme poses. Thier architecture consists of a face boundry transformer network and a face sythesis network. The boundry transformer network uses t(1) the encoder $En_{b1}$ encodes the target's boundry image $b_t$ to $v_t$, (2) two networks $P$ and $E$ estimate the pose vector $p_s$ and expression vector $e_s$ using the source's boundry image $b_s$, and (3) the concatenation of $e_s$, $p_s$, and $v_t$ are passed to the decoder $De_b$ which generates $b_g$, the boundry image of the target witht he source's expression and pose. To train this network, the authors use a combination of L1 loss on images with labeled expression vectors, and conditional regresson loss on randomly generated $e$ and $p$ on a given $v$ to cover unseen poses and expressions.
	
	%summarize and place in category by date (many-2-one...,date)
	\cite{zhou2019dance}
	\cite{siarohin2018deformable}
	\cite{balakrishnan2018synthesizing}
	\cite{de2019conditional}
	\cite{ma2018disentangled}
	\cite{zhu2019progressive}
	\cite{lee2019metapix}
